Enabling an OpenStack-based cloud on top of RISC-V hardware

The European Union's technological sovereignty strategy centers around the RISC-V Instruction Set Architecture, with the European Processor Initiative leading efforts to build production-ready processors. Focusing on realizing a functional RISC-V cloud ecosystem, the Vitamin-V European project developed an OpenStack cluster utilizing genuine hardware. In this poster, we detail the efforts done in porting and setting up the cluster and the many software services required by OpenStack to properly run on real hardware. In this poster, we detail our efforts on building an minimal viable prototype OpenStack cluster using real hardware. The cluster is almost functional, and we expect it to be complete in the next few months.

==> abstract.tex <==


As a part of the \footnote{\label{note1}Omitted for blind review} project, our team has dedicated the last year developing a functional OpenStack cluster utilizing real hardware instead of emulators. Initially, the core of our building and deploying platform
was based on QEMU, however, after a few months we switched to real hardware due to the superior performance and reliability.

As the hardware platform we are using a RISC-V development board by Sipeed, the Lichee PI 4A owing to their balanced pricing and capabilities. More specifically, the utilized development platform provides a TH1520 RISC-V CPU (4 Threads), 16GB of RAM, 128GB storage. In addition it also provides a dual Gigabit Ethernet a feature particularly interesting when building an OpenStack cluster.

Due to the novelty of both RISC-V chips and OS (linux), building the cluster from scracth presented several challenges at different levels: operating system, to distribution and packages. To run openstack, we built a custom linux kernel to include missing modules needed by OpenStack (e.g., openvswitch) and removed unnecessary modules to make the custom kernel fit the partition. The default linux distribution is a version of debian by Sipeed target their repositories which does not provide all Debian packages, specially most development packages were missing. Regarding deployment and cluster management we used ansible which was not part of the Sipeed Debian repository. 

As the project advanced, the oficial Debian repositories increased their packages coverage up to 95\% of the packages build for RISC-V, easing deployment procedures. We decided to switch to all packages to official debian, and only use the Sipeed software for building the custom kernel. 

Another challenge involved updating the operating system on all nodes simultaneously. We decided to use Ansible as the deployment tool. Ansible is a popular tool among administrators for deploying and configuring large clusters to ensure reproducibility. We also explored using Devstack and Kolla to deploy and configure OpenStack. However, both options download specific versions of packages and dependencies, which turned into many compilation issues on RISC-V


The current OpenStack cluster comprises 6 Lichee PI4A boards, each of which, taking the following roles: 1 controller node, 4 compuute nodes, and 1 board serving files. The controller node runs the dashboard to launch new instances and set up machines. It also runs other services such as database, message queue, identity, and image services, along with the server side of Compute and Network. The compute and network services inform the hypervisor regarding the \ac{VM}s configuration. The configuration is set on the client side.


